Hyperbolic VAE via Latent Gaussian Distributions

We propose a Gaussian manifold variational auto-encoder (GM-VAE) whose latent space consists of a set of Gaussian distributions. It is known that the set of the univariate Gaussian distributions with the Fisher information metric form a hyperbolic space, which we call a Gaussian manifold. To learn the VAE endowed with the Gaussian manifolds, we propose a pseudo-Gaussian manifold normal distribution based on the Kullback-Leibler divergence, a local approximation of the squared Fisher-Rao distance, to define a density over the latent space. In experiments, we demonstrate the efficacy of GM-VAE on two different tasks: density estimation of image datasets and environment modeling in model-based reinforcement learning. GM-VAE outperforms the other variants of hyperbolic- and Euclidean-VAEs on density estimation tasks and shows competitive performance in model-based reinforcement learning. We observe that our model provides strong numerical stability, addressing a common limitation reported in previous hyperbolic-VAEs.

==> algorithm/enc_algo.tex <==
\begin{algorithm}[H]
\hsize=\textwidth %
% \setstretch{1.3}
\caption{Encoder}
%\hspace*{\algorithmicindent} 
 \textbf{Input}  Input data $\rvx$, Encoding layers $\textrm{Enc}(\cdot)$ \\
 \textbf{Output} $(\alpha, \beta) \in \mathcal{G}_c$, $\gamma \in \mathbb{R}_{>0}$ \\
\begin{algorithmic}[1]
\STATE $\alpha, \beta, \gamma = \textrm{Enc}(\rvx)$
%\STATE $\tilde{\rvv}, \gamma^2 = \textrm{Enc}(\rvx)$ \COMMENT{$\tilde{\rvv} \in \mathcal{E}$}
%\STATE ${\rvv} = \exp_{\boldsymbol{0}_\mathcal{L}}^c(f(\tilde{\rvv}))$ \COMMENT{$\rvv \in \mathcal{L}^2_c$}
%\STATE ${(\alpha, \beta)} = T_c({\rvv}) $ \COMMENT{$(\alpha, \beta) \in \mathcal{G}_c$}
\STATE \textbf{return} $(\alpha, \beta), \gamma$
\end{algorithmic}
\label{alg:enc}
\end{algorithm}

==> appendices/06_NumericalStability.tex <==
\section{Numerical Stability}
\label{apx:numerical_stability}
We conduct an analysis of the numerical stability of the PGM normal distribution compared to the HWN and Poincar\'e normal. 
During the density estimation experiment, the HWN VAE and Poincar\'e VAE are often shown to be numerically unstable and fail to run in binarized-Breakout. Similar observations have been reported in several previous works ~\citep{mathieu19, fhnn, MVAE}.

The hyperbolic wrapped normal uses the exponential map when transforming the output of the encoder to the Lorentz model and during the sampling, as described in \autoref{eq:wrapped_normal}.
The overlapped Lorentz model exponential map often causes an overflow due to the hyperbolic functions in the exponential map such as $\cosh$ and $\sinh$.
Note that the hyperbolic functions exponentially grow with the positive input value.

In the training of Poincar\'e VAE, the KL divergence between the variational distribution and the prior distribution needs to be approximated by the log-probability of the samples due to the absence of closed-form KL divergence in Poincar\'e normal.
To compute the log probability of a given sample, the distance between two Poincar\'e disk model points, the sample and the Fr\'echet mean of the distribution needs to be calculated, where the distance function of the Poincar\'e disk model is defined as:
\begin{equation}
    d^c_{\mathcal{P}}(\rvx, \rvy) = \frac{1}{\sqrt{c}} \cosh^{-1}\left(1 + 2c \frac{\Vert \rvx - \rvy \Vert^2}{(1 - c\Vert \rvx \Vert^2)(1 - c\Vert \rvy \Vert^2)} \right),
\end{equation}
where $\Vert \cdot \Vert$ is the Euclidean norm.
The denominator term is unstable when $\Vert \rvx \Vert$ or $\Vert \rvy \Vert$ is close to value $\frac{1}{\sqrt{c}}$, which occurs when $\rvx$ and $\rvy$ are near the border of the Poincar\'e disk.

PGM normal, on the other hand, the KL divergence between an arbitrary PGM normal and $\mathcal{K}_c(\boldsymbol{0}, I, I)$, which is the only operation used during the training of GM-VAE, can be stably computed using the log-covariance.
For example, the KL divergence between a univariate Gaussian distribution $\mathcal{N}(\mu, \sigma)$ and the prior distribution mentioned above written as \autoref{eq:kl_divergence} can be computed with $\log \sigma^2$.
The KL divergence between two Gamma distributions, $\textrm{Gamma}(a_1, b_1)$ and $\textrm{Gamma}(a_2, b_2)$, written as:
\begin{equation}
    \KL(\textrm{Gamma}(a_1, b_1) \parallel \textrm{Gamma}(a_1, b_1)) = a_2 \log \frac{b_1}{b_2} - \ln \frac{\Gamma(a_1)}{\Gamma(a_2)} + (a_1 - a_2) \psi(a_1) - (1 - \frac{b_2}{b_1}) a_1,
\end{equation}
where $\psi$ is the digamma function, can be stablly computed using $\log b_1$ when $b_1$ is large due to small $\beta$ and $\gamma$ in the factorization \autoref{eq:factorization}.



==> appendices/Isometries.tex <==
\section{Operations of the Hyperbolic Spaces}
\label{apx:geometric_transformations}

\subsection{Isometries}
In this section, we derive the isometries between the two-dimensional hyperbolic models, the Lorentz model, the Poincar\'e disk model and the Gaussian manifold with arbitrary curvatures.
Isometry between the Poincar\'e disk model and the Lorentz model $T_{\mathcal{L}_c \rightarrow \mathcal{P}_c}: \mathcal{L}_c \rightarrow \mathcal{P}_c$ is computed as:
\begin{equation*}
    T_{\mathcal{L}_c \rightarrow \mathcal{P}_c}((t, x, y)) = \left(\frac{x}{\sqrt{c}t + 1}, \frac{y}{\sqrt{c}t + 1}\right),
\end{equation*}
and the inverse is:
\begin{equation}
    T^{-1}_{\mathcal{L}_c \rightarrow \mathcal{P}_c}((x, y)) \left( \frac{1 + (x^2 + y^2)c}{\sqrt{c} (1 - (x ^2 + y^2)c)}, \frac{2x}{1 - (x ^2 + y^2)c}, \frac{2y}{1 - (x ^2 + y^2)c} \right).
\end{equation}

Isometry between the Gaussian manifold and the Poincar\'e disk model $T_{\mathcal{P}_c \rightarrow \mathcal{U}_c}: \mathcal{P}_c \rightarrow \mathcal{U}_c$ is computed as:
\begin{equation*}
    T_{\mathcal{P}_c \rightarrow \mathcal{G}_c}(x, y) = \left( \frac{-2y}{(\sqrt{c}x - 1)^2 + y^-2c}, \frac{1 - (x^2 + y^2)c}{(\sqrt{c}x - 1)^2 + y^-2c} \right), 
\end{equation*}
and the inverse is:
\begin{equation}
     T^{-1}_{\mathcal{P}_c \rightarrow \mathcal{G}_c}(x, y) \left( \frac{\sqrt{c}x^2 + (y^2 - 1) / \sqrt{c}}{cx^2 + (y + 1)^2}, \frac{-2x}{cx^2 + (y + 1)^2} \right).
\end{equation}

Finally, the isometry between the Gaussian manifold and the Lorentz model $T_{\mathcal{L}_c \rightarrow \mathcal{G}_c}$ can be derived by composing $T_{\mathcal{L}_c \rightarrow \mathcal{P}_c}$ and $T_{\mathcal{P}_c \rightarrow \mathcal{G}_c}$ as:
\begin{equation*}
    T_{\mathcal{L}_c \rightarrow \mathcal{G}_c}(t, x, y) = \left( \frac{-y}{\sqrt{c}(t-x)}, \frac{1}{\sqrt{c}(t - x)} \right), 
\end{equation*}
and the inverse is:
\begin{equation}
    T^{-1}_{\mathcal{L}_c \rightarrow \mathcal{G}_c}(x, y) = \left( \frac{1 + cx^2 + y^2}{2\sqrt{c}y}, \frac{-1 + cx^2 + y^2}{2\sqrt{c}y}, -\frac{x}{y}\right).
\end{equation}

We then empirically show that the isometries preserve the distance between the points when transformed to other models.
We randomly sampled 1,000 pairs of Gaussian manifold points with range of $\mu \in [-100, 100]$ and $\sigma \in [0, 100]$. We report the average difference in the distance for each pair before the transformation and after the transformation. We vary the curvature value from 0.25 to 2.
For the Gaussian manifold, we use the following distance function for arbitrary curvature:
\begin{equation*}
    d_{\mathcal{U}_c}((x_1, y_1), (x_2, y_2)) = \frac{1}{\sqrt{c}}\log \frac{\sqrt{c(x_1 - x_2)^2 + (y_1 + y_2)^2 } + \sqrt{c(x_1 - x_2)^2 + (y_1 - y_2)^2}}{\sqrt{c(x_1 - x_2)^2 + (y_1 + y_2)^2} - \sqrt{c(x_1 - x_2)^2 + (y_1 - y_2)^2}}.
\end{equation*}
\autoref{tab:isometry_validation} shows that the proposed isometries well-preserve the distances.


\input{tables/isometry_validation}

% Distance metric in the Lorentz model:
% \begin{equation*}
%     d^c_{\mathbb{L}}((t_1, x_1, y_1), (t_2, x_2, y_2)) = \sqrt{-2\left(\frac{1}{c} -t_1t_2 + x_1x_2 + y_1y_2\right)}
% \end{equation*}

\subsection{the Lorentz model operations}
The $n$-dimensional Lorentz model with curvature $-c$ is $\mathcal{L}^n_c$ where the manifold is $\{\rvx \in \R^{n+1} \mid \langle \rvx, \rvx \rangle_{\mathcal{L}_c} = -\frac{1}{c}\}$, where $\langle \rvx, \rvy \rangle_{\mathcal{L}_c}$ is the Lorentzian product computed as $\langle \rvx, \rvy \rangle_{\mathcal{L}_c} = -\rvx_0 \rvy_0 + \sum_{i=1}^n \rvx_i \rvy_i$.
% The Lorentzian norm is computed as $\Vert \rvv \Vert_{\mathbb{L}_c} = \s$
The exponential map of the Lorentz model is defined as:
\begin{equation}
% \label{eq:wrapped_normal}
    \exp_{\rvx}^c(\rvv) = \cosh(\alpha)\rvx + \sinh(\alpha) \frac{\rvv}{\alpha},
\end{equation}
and the log map of the Lorentz model is defined as:
\begin{equation}
    \log_{\rvx}^c(\rvy) = \frac{\cosh^{-1}(\beta)}{\sqrt{\beta^2 - 1}} (\rvy - \beta \rvx),
\end{equation}
where $\alpha = \sqrt{c\langle \rvv, \rvv \rangle_{\mathbb{L}_c}}$ and $\beta = -c\langle \rvx, \rvy \rangle_{\mathbb{L}_c}$.

==> appendices/LatentAnalysis.tex <==
\section{Latent Space Analysis}
\label{apx:latent_space_analysis}
In this section, we provide additional visualizations of the learned representations of GM-VAE.
\autoref{fig:MNIST_tsne_euc} shows the t-SNE visualization of the Euclidean VAE learned on binarized-MNIST.
\autoref{fig:MNIST_mu} shows the interpolation results of the binarized-MNIST representations along the $\mu$ axis, by changing the value of $\alpha$ on three dimensions and fixing all the other values including $\beta$.
\autoref{fig:MNIST_latents} and \autoref{fig:Breakout_latents} show the latent representations from all the dimensions with binarized-MNIST and binarized-Breakout respectively.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/images/tsne_EuclideanNormal.pdf}
    \caption{t-SNE visualization with representations learned from Euclidean-VAE.}
    \label{fig:MNIST_tsne_euc}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/images/mnist_mu_interpolation.png}
    \caption{Interpolation results of the representations learned from GM-VAE along the $\mu$ axis.}
    \label{fig:MNIST_mu}
\end{figure}

\input{figures/Breakout_latents}
\input{figures/MNIST_latents}


==> figures/Breakout_analysis.tex <==
\begin{figure}[t!]
    \centering
    %\hfill
    \begin{subfigure}[t]{.6\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_interpolation.png}
        \caption{Latent traversal of representations.}
        \label{fig:Breakout_dim}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/hierarchy_Breakout.pdf}
        \caption{Hierarchy in the data.}
    \end{subfigure}
    %\hfill
    \caption{Analysis of the latent space learned from GM-VAE with the binarized-Breakout. (a) Reconstructing the representations, along the gray line, shows a similar hierarchical structure, where (b) the hierarchy between the images is expressed as the dotted line. }
    \label{fig:Breakout_analysis}
\end{figure}

==> figures/Breakout_latents.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_00.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_01.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_02.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_03.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_04.png}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_05.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_06.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_07.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_08.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_09.png}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_10.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_11.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_12.png}
    \end{subfigure}
    \begin{subfigure}[t]{.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/breakout_latents/latent_Breakout_13.png}
    \end{subfigure}
    \\
    \caption{The binarized-Breakout representations learned from GM-VAE.}
    \label{fig:Breakout_latents}
\end{figure}

==> figures/MNIST_analysis.tex <==
\begin{figure}[b!]
    \centering
    \begin{subfigure}[t]{.45\linewidth}
        \centering
        \includegraphics[width=0.8\linewidth]{figures/images/mnist_tsne_PGM.png}
        \caption{t-SNE visualization.}
        \label{fig:MNIST_tsne}
    \end{subfigure}
    %\hspace{1mm}
    %\hfill
    \begin{subfigure}[t]{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_interpolation.png}
        \caption{Latent traversal of representations.}
        \label{fig:MNIST_interpolation}
    \end{subfigure}
    \caption{Analysis of the learned latent space of GM-VAE with binarized-MNIST. (a) t-SNE visualization of the representation with respect to the class labels.
    %where a comparison with $\mathcal{E}$-VAE is available in \autoref{apx:latent_mnist}. 
    (b) Increasing the value of $\beta$, along the gray line, results in an increasing degree of uncertainty in the reconstructed images. }
    \label{fig:MNIST_analysis}
\end{figure}

==> figures/MNIST_latents.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_00.png}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_01.png}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_02.png}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_03.png}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_04.png}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_05.png}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_06.png}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mnist_latents/latent_MNIST_07.png}
    \end{subfigure}
    \caption{The binarized-MNIST representations learned from GM-VAE.}
    \label{fig:MNIST_latents}
\end{figure}

==> figures/gmvae_architecture.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/images/gm_vae.pdf}
    \caption{An exemplar architecture of GM-VAE. The illustration shows the architecture of GM-VAE which sets the latent space to a three-dimensional diagonal Gaussian manifold. The encoder outputs parameters of the PGM normal, which are the points of the Gaussian manifold. The arrow refers to the sampling process. The decoder reconstructs data from the samples. %GM-VAE is trained to maximize ELBO, including the log-likelihood of the reconstructed data.
    }
    \label{fig:overall_structure}
\end{figure}

==> figures/hyperbolic_isometries.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{.32\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{figures/images/halfplane.png}
        \caption{Poincar\'e half-plane model}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/poincare.png}
        \caption{Poincar\'e disk model}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/lorentz.png}
        \caption{Lorentz model}
    \end{subfigure}
    \hfill
    \caption{Caption}
    \label{fig:hyperbolic_isometries}
\end{figure}

==> figures/image_hierarchy.tex <==
\begin{figure}[t!]
    \centering
    % \vspace*{0.3cm}
    % \vskip -0.1in
    \begin{subfigure}[t!]{.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/cub.pdf}
        \caption{CUB}
    \end{subfigure}
    \hspace{15.mm}
    \begin{subfigure}[t!]{.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/oxford.pdf}
        \caption{Oxford102}
    \end{subfigure}
    \caption{
    Sample images from CUB and Oxford102 datasets with exemplary hierarchical relationships from the biological classification between images.
    }
    \label{fig:image_hierarchy}
\end{figure}

==> figures/world_model_analysis.tex <==
\begin{figure}[b!]
    \centering
    \vskip -0.1in
    \includegraphics[width=.55\linewidth]{figures/images/hwm_analysis.png}
    \caption{
    The dots from yellow to purple represent the latent states from the world model in the Atari2600 Breakout with decreasing rewards. 
    Along the red geodesic dashed line passing, we sample for images to visualize the learned representations. As the sample shows, we can observe a hierarchical structure at different stages of the game along the geodesic.
    }
    \vspace*{0.7cm}
    \label{fig:world_model_analysis}
\end{figure}

==> tables/float_density_estimation.tex <==
% \begin{table}[t!]
%     \centering
%     \caption{Density estimation on real-world datasets. $d$ denotes the latent dimension. We report the negative test log-likelihoods of average 10 runs for binarized-MNIST and binarized-Omniglot, and an average 5 runs for binarized-Breakout with the 95\% confidence interval. N/A in the log-likelihood indicates that the results are not available due to the failure of all runs, and N/A in the standard deviation indicates that the results are not available due to failures of some runs.}
%     \resizebox{\textwidth}{!}
%     {%
%     \begin{tabular}{l l r r r r r r}
%         \toprule
%          &\multicolumn{1}{c}{$d$}&\multicolumn{1}{c}{$\mathcal{E}$-VAE}&\multicolumn{1}{c}{$\mathcal{L}$-VAE}&\multicolumn{1}{c}{$\mathcal{P}$-VAE} &\begin{tabular}{@{}c@{}}GM-VAE\\($c=1$)\end{tabular}&\begin{tabular}{@{}c@{}}GM-VAE \\ ($c=1/2$)\end{tabular}&\begin{tabular}{@{}c@{}}GM-VAE \\ ($c=3/2$)\end{tabular}\\
%          \midrule
%          \multirow{3}{*}{MNIST} 
%          &10%&$79.72_{\pm 0.13}$&$80.01_{\pm 0.23}$&N/A\\
%          &20%&$74.49_{\pm 0.42}$&$73.59_{\pm 0.21}$&N/A\\
%          &30%&$73.56_{\pm 0.25}$&$73.56_{\pm 0.16}$&N/A\\
%          \midrule
%          \multirow{3}{*}{Omniglot} 
%          &10%&$135.74_{\pm 0.52}$&$135.93_{\pm 0.90}$&%$-129.72_{\textrm{N/A}}$
%          &20%&$121.00_{\pm 0.34}$&$120.44_{\pm 0.41}$&N/A
%          &30%&$118.82_{\pm 0.44}$&$117.82_{\pm 0.32}$&N/A
%          \midrule
%          \multirow{3}{*}{Breakout}
%          &24&$50.37_{\pm.46}$&$50.82_{\textrm{N/A}}$&\textrm{N/A}& $\pmb{49.35_{\pm.67}}$&$50.82_{\pm.92}$&$49.88_{\pm.51}$\\
%          &28&$48.07_{\pm.20}$&$48.74_{\textrm{N/A}}$&\textrm{N/A}&$47.01_{\pm.31}$&$48.31_{\pm.47}$&$\pmb{46.82_{\pm.77}}$\\
%          &32&$48.06_{\pm.18}$&$48.64_{\textrm{N/A}}$&\textrm{N/A}&$47.04_{\pm.23}$&$48.13_{\pm.30}$&$\pmb{46.88_{\pm.25}}$\\
%          \bottomrule
%     \end{tabular}%
%     }
%     \label{tab:float_density_estimation}
% \end{table}
\begin{table}[t!]
    \centering
    \caption{TODO}
    \resizebox{\textwidth}{!}
    {%
    \begin{tabular}{l l r r r r r r}
        \toprule
         &\multicolumn{1}{c}{$d$}&\multicolumn{1}{c}{$\mathcal{E}$-VAE}&\multicolumn{1}{c}{$\mathcal{L}$-VAE}&\multicolumn{1}{c}{$\mathcal{P}$-VAE} &\begin{tabular}{@{}c@{}}GM-VAE \\($c=1$)\end{tabular}&\begin{tabular}{@{}c@{}}GM-VAE \\ ($c=1/2$)\end{tabular}&\begin{tabular}{@{}c@{}}GM-VAE \\ ($c=3/2$)\end{tabular}\\
         \midrule
         \multirow{3}{*}{MNIST} 
         &10&$79.72_{\pm 0.13}$&$80.01_{\pm 0.23}$&N/A&$80.38_{\pm 0.14}$&$80.07_{\pm 0.21}$&$80.50_{\pm 0.17}$\\
         &20&$74.49_{\pm 0.42}$&$73.59_{\pm 0.21}$&N/A&$73.52_{\pm 0.13}$&$73.52_{\pm 0.34}$&$73.45_{\pm 0.21}$\\
         &30&$73.56_{\pm 0.25}$&$73.56_{\pm 0.16}$&N/A&$73.37_{\pm 0.08}$&$73.19_{\pm 0.09}$&$73.51_{\pm 0.14}$\\
         \midrule
         \multirow{3}{*}{Omniglot} 
         &10&$135.74_{\pm 0.52}$&$135.93_{\pm 0.90}$&$-129.72_{\textrm{N/A}}$&$133.91_{\pm 0.29}$&$135.01_{\pm 0.43}$&$133.35_{\pm 0.43}$\\
         &20&$121.00_{\pm 0.34}$&$120.44_{\pm 0.41}$&N/A&$118.58_{\pm 0.45}$&$119.18_{\pm 0.52}$&$118.78_{\pm 0.62}$\\
         &30&$118.82_{\pm 0.44}$&$117.82_{\pm 0.32}$&N/A&$117.84_{\pm 0.25}$&$117.85_{\pm 0.18}$&$118.22_{\pm 0.42}$\\
         \midrule
         \multirow{3}{*}{Breakout}
         &24&$50.20_{\pm 0.45}$&N/A&N/A&$50.17_{\pm 0.81}$&$50.57_{\pm 0.31}$&NaN\\
         &28&$48.21_{\pm 0.27}$&N/A&N/A&$47.58_{\pm 0.44}$&$48.42_{\pm 0.35}$&NaN\\
         &32&$47.84_{\pm 0.32}$&N/A&N/A&$47.37_{\pm 0.30}$&$48.47_{\pm 0.23}$&NaN\\
         \bottomrule
    \end{tabular}%
    }
    \label{tab:float_density_estimation}
\end{table}

==> tables/geometric_transformations.tex <==
\begin{table*}[t!]
    \centering
    \caption{Ablation study on the geometric transformations of GM-VAE. Vanilla denotes the models without the geometric transformations, and Geo denotes the models with the geometric transformations. The geometric transformations enhance the generalization performance in most cases.}
    \label{tab:architecture_ablation}
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{l l r r r r r r}
        \toprule
        &&\multicolumn{2}{c}{$c=1$}&\multicolumn{2}{c}{$c=1/2$}&\multicolumn{2}{c}{$c=3/2$}\\
        \cmidrule(l){3-4} \cmidrule(l){5-6}\cmidrule(l){7-8}
         &\multicolumn{1}{c}{$d$}&\multicolumn{1}{c}{Vanilla}&\multicolumn{1}{c}{Geo}&\multicolumn{1}{c}{Vanilla}&\multicolumn{1}{c}{Geo}&\multicolumn{1}{c}{Vanilla}&\multicolumn{1}{c}{Geo}\\
         \midrule
         \multirow{3}{*}{MNIST}
         &10&$\pmb{80.28_{\pm.17}}$&$80.34_{\pm.30}$&$80.28_{\pm.19}$&$\pmb{80.10_{\pm.20}}$&$\pmb{80.38_{\pm.20}}$&$\pmb{80.38_{\pm.18}}$\\
         %&16&$76.24_{\pm.52}$& $\pmb{73.47_{\pm.13}}$& $75.37_{\pm.57}$& $\pmb{73.95_{\pm.30}}$& $76.36_{\pm.67}$& $\pmb{73.72_{\pm.18}}$\\
         &20&$75.33_{\pm.75}$& $\pmb{73.27_{\pm.22}}$& $74.94_{\pm.58}$& $\pmb{73.31_{\pm.29}}$& $75.74_{\pm.70}$& $\pmb{73.28_{\pm.19}}$\\
         %&24&$75.04_{\pm.54}$& $\pmb{73.24_{\pm.17}}$& $74.97_{\pm.71}$& $\pmb{73.49_{\pm.28}}$& $75.41_{\pm.62}$& $\pmb{73.72_{\pm.09}}$\\
         &30&$74.63_{\pm.08}$&$\pmb{73.49_{\pm.13}}$&$74.48_{\pm.50}$&$\pmb{73.35_{\pm.16}}$&$75.05_{\pm.43}$&$\pmb{73.55_{\pm.22}}$\\
         %&40&$74.48_{\pm.38}$&$\pmb{73.66_{\pm.08}}$&$74.16_{\pm.29}$&$\pmb{73.18_{\pm.07}}$&$74.74_{\pm.19}$&$\pmb{73.75_{\pm.11}}$\\
         \midrule
         \multirow{3}{*}{Omniglot}
         &10&$135.12_{\pm.35}$&$\pmb{134.01_{\pm.28}}$&$135.47_{\pm.24}$&$\pmb{135.20_{\pm.21}}$&$134.69_{\pm.37}$&$\pmb{133.79_{\pm.30}}$\\
         %&16&$123.40_{\pm.42}$& $\pmb{122.31_{\pm.30}}$& $\pmb{123.56_{\pm.18}}$& $123.65_{\pm.23}$& $123.62_{\pm.54}$& $\pmb{122.05_{\pm.21}}$\\
         &20&$122.24_{\pm.67}$& $\pmb{118.79_{\pm.53}}$& $121.10_{\pm.59}$& $\pmb{118.73_{\pm.39}}$& $122.44_{\pm.61}$& $\pmb{119.03_{\pm.57}}$\\
         %&24&$121.05_{\pm.30}$& $\pmb{117.95_{\pm.19}}$& $120.44_{\pm.33}$& $\pmb{118.48_{\pm.28}}$& $121.39_{\pm.64}$& $\pmb{117.92_{\pm.57}}$\\
         &30&$120.85_{\pm.33}$&$\pmb{117.97_{\pm.35}}$&$119.48_{\pm.56}$&$\pmb{117.70_{\pm.47}}$&$121.23_{\pm.68}$&$\pmb{117.95_{\pm.37}}$\\
         %&40&$119.72_{\pm.48}$&$\pmb{118.27_{\pm.40}}$&$118.67_{\pm.36}$&$\pmb{117.65_{\pm.53}}$&$120.54_{\pm.63}$&$\pmb{118.92_{\pm.40}}$\\
         \midrule
         \multirow{3}{*}{Breakout}
         &24&$51.69_{\pm.20}$&$\pmb{49.35_{\pm.67}}$& $51.04_{\pm.72}$& $\pmb{50.82_{\pm.92}}$&$51.57_{\pm.50}$& $\pmb{49.88_{\pm.51}}$\\
         &28&$49.56_{\pm.69}$&$\pmb{47.01_{\pm.31}}$&$49.51_{\pm.51}$& $\pmb{48.31_{\pm.47}}$&$49.45_{\pm.63}$&$\pmb{46.82_{\pm.77}}$\\
         &32&$49.45_{\pm.29}$&$\pmb{47.04_{\pm.23}}$&$49.03_{\pm.38}$& $\pmb{48.13_{\pm.30}}$&$49.07_{\pm.54}$&$\pmb{46.88_{\pm.25}}$\\
         \bottomrule
    \end{tabular}
    %}
\end{table*}


==> tables/hyperbolic_distributions.tex <==
\begin{wraptable}{r}{.5\textwidth}
    \centering
    \vskip -0.18in
    \caption{A comparison of the PGM normal (PGM-$\mathcal{N}$) with HWN and Poincar\'e normal (Poincar\'e-$\mathcal{N}$).
    Geometry denotes whether the distribution utilizes the geometric structure. %, i.e., geodesic distance.
    Tractable KL indicates whether the distribution has a closed-form KL divergence.
    }
    \label{tab:distribution_related_work}
    % \vskip 0.1in
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c}
        \toprule
        % uncertainty, closed-form update
        & Sampling
        %$\bm\alpha$
        & Geometry
        %in $q_u(\mTheta^{(u)})$
        & Tractable KL
        \\
        \midrule
        HWN & \footnotesize{low-cost}  & $\times$ & $\times$ \\
        Poincar\'e $\mathcal{N}$ & \footnotesize{expensive} & $\bigcirc$ & $\times$ \\
        PGM-$\mathcal{N}$ & \footnotesize{low-cost}  & $\bigcirc$ & $\bigcirc$ \\
        \bottomrule
    \end{tabular}
    }
\end{wraptable}

==> tables/image_split.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{c | c c c}
         \toprule
         Split & Breakout & Oxford102 & CUB \\
         \midrule
         Train & 80,000 & 5,120 & 4,795 \\
         Validation & 9,503  & 1,228 & 1,199 \\
         Test & 9,934 & 1,025 & 5,794 \\
         \bottomrule
    \end{tabular}
\end{table}


==> tables/isometry_validation.tex <==
\begin{table}[h!]
    \centering
    \caption{Validation of the proposed isometries between the hyperbolic models.}
    \label{tab:isometry_validation}
    \begin{tabular}{r c c c}
        \toprule
        $c$
        & $T_{\mathcal{P}_c \rightarrow \mathcal{L}_c}$
        & $T_{\mathcal{G}_c \rightarrow \mathcal{P}_c}$
        & $T_{\mathcal{G}_c \rightarrow \mathcal{L}_c}$
        \\
        \midrule
        0.25 & $5.72\textrm{e}{-13}$& $1.50\textrm{e}{-13}$& $4.76\textrm{e}{-13}$\\
        0.50 & $8.41\textrm{e}{-13}$& $3.10\textrm{e}{-13}$& $6.23\textrm{e}{-13}$\\
        1.00& $7.84\textrm{e}{-13}$& $4.22\textrm{e}{-13}$& $4.88\textrm{e}{-13}$ \\
        1.50& $3.22\textrm{e}{-12}$& $2.51\textrm{e}{-12}$& $8.30\textrm{e}{-13}$ \\
        2.00& $1.89\textrm{e}{-12}$& $1.20\textrm{e}{-12}$& $8.86\textrm{e}{-13}$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/model_based_rl.tex <==
\begin{table}[b!]
    \centering
    %\vskip -0.2in
    \caption{
    Model-based RL results on the 6 games of the Atari2600 environment. 
    We compare the methods of using Euclidean, discrete, and hyperbolic latent space.
    We report averaged rewards over 4 runs. 
    The best reward for each game is bolded.
    }
    \vskip 0.1in
    %\resizebox{\textwidth}{!}{%
    \begin{tabular}{c r r r r}
        \toprule
         Latent space & Euc. & Disc. & Hyp. & $\delta-$H \\
         \midrule
         Breakout & $\mathbf{329.0}$ & 256.8 & 319.3 & 0.12 \\
         Alien & 3412.5 & 3120.0 & $\mathbf{3485.0}$ & 0.14 \\  
         Zaxxon & 34275 & 38825 & $\mathbf{38950}$ & 0.14 \\
         Ice Hockey & $\mathbf{25.50}$ & 11.80 & 20.75 & 0.14 \\
         \midrule
         Freeway & 32.8 & $\mathbf{33.0}$ & $\mathbf{33.0}$ & 0.38 \\
         Krull & 53290 & 36135 & $\mathbf{66185}$ &  0.38 \\
         \bottomrule
    \end{tabular}%
    %}
    \label{tab:rl_results}
\end{table}
